Alchemist: Parametric Control of Material Properties with Diffusion Models

We propose a method to control material attributes of objects like roughness, metallic, albedo, and transparency in real images. Our method capitalizes on the generative prior of text-to-image models known for photorealism, employing a scalar value and instructions to alter low-level material properties. Addressing the lack of datasets with controlled material attributes, we generated an object-centric synthetic dataset with physically-based materials. Fine-tuning a modified pre-trained text-to-image model on this synthetic dataset enables us to edit material properties in real-world images while preserving all other attributes. We show the potential application of our model to material edited NeRFs.

==> figures/tex/albedo_test.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=1.0\linewidth]{figures/source/albedo_test.pdf}
\caption{\textbf{Albedo test results.} Comparison of our method to InstructPix2Pix prompt-only method trained on our data (Baseline) for editing albedo on held-out synthetic data for different strengths.}
\label{fig:albedo_test}
\end{figure*}

==> figures/tex/metallic_test.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=1.0\linewidth]{figures/source/metallic_test.pdf}
\caption{\textbf{Metallic test results.} Comparison of our method to InstructPix2Pix prompt-only method trained on our data (Baseline) for editing metallic attribute on held-out synthetic data for different strengths.}
\label{fig:metallic_test}
\end{figure*}

==> figures/tex/roughness_test.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=1.0\linewidth]{figures/source/roughness_test.pdf}
\caption{\textbf{Roughness test results.} Comparison of our method to InstructPix2Pix prompt-only method trained on our data (Baseline) for editing roughness on held-out synthetic data for different strengths.}
\label{fig:roughness_test}
\end{figure*}

==> figures/tex/transparency_test.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=1.0\linewidth]{figures/source/transparency_test.pdf}
\caption{\textbf{Transparency test results.} Comparison of our method to InstructPix2Pix prompt-only method trained on our data (Baseline) for editing transparency on held-out synthetic data for different strengths.}
\label{fig:transparency_test}
\end{figure*}
